Quantum Prometheus: Defying Overhead with Recycled Ancillas in Quantum Error Correction

Quantum error correction (QEC) is crucial for ensuring the reliability of quantum computers. However, implementing QEC often requires a significant number of qubits, leading to substantial overhead. One of the major challenges in quantum computing is reducing this overhead, especially since QEC codes depend heavily on ancilla qubits for stabilizer measurements. In this work, we propose reducing the number of ancilla qubits by reusing the same ancilla qubits for both X- and Z-type stabilizers. This is achieved by alternating between X and Z stabilizer measurements during each half-round, cutting the number of required ancilla qubits in half. This technique can be applied broadly across various QEC codes, we focus on rotated surface codes only and achieve nearly \(25\%\) reduction in total qubit overhead. We also present a few use cases where the proposed idea enables the usage of higher-distance surface codes at a relatively lesser qubit count. Our analysis shows that the modified approach enables users to achieve similar or better error correction with fewer qubits, especially for higher distances (\(d \geq 13\)). Additionally, we identify conditions where the modified code allows for extended distances (\(d + k\)) while using the same or fewer resources as the original, offering a scalable and practical solution for quantum error correction. These findings emphasize the modified surface code's potential to optimize qubit usage in resource-constrained quantum systems.

==> 1_introduction_old.tex <==
\section{Introduction} \label{sec:introduction}

Quantum Error Correction (QEC) is a fundamental requirement for the reliable operation of quantum computers. In the delicate environment of quantum computation, where information is encoded in fragile quantum states, even the slightest interaction with the surrounding environment can induce errors that compromise computational accuracy~\cite{mouloudakis2021entanglement}. Quantum systems are particularly vulnerable to two primary types of errors: bit-flip and phase-flip errors. Unlike classical systems, which primarily contend with bit-flip errors, quantum systems face the additional complexity of phase-flip errors due to the unique properties of quantum information. Traditional error correction techniques, as applied in classical systems, are ineffective for quantum data because of the constraints imposed by the no-cloning theorem and the disruptive nature of quantum measurement~\cite{wootters2009no, von2018mathematical}. This intrinsic vulnerability of quantum states underscores the necessity for specialized QEC techniques tailored to the quantum realm.

To counteract these errors, QEC introduces various stabilizer codes, which employ ancillary, or ``ancilla," qubits to measure and correct errors without disturbing the encoded quantum information. However, the robustness of QEC comes at a significant cost: the need for numerous ancilla qubits, which imposes substantial overhead on quantum systems and presents a major barrier to scalable quantum computation. 

Surface codes~\cite{dennis2002topological} address both bit and phase errors by using a two-dimensional qubit layout. Such an approach makes them a frontrunner for near-term fault-tolerant quantum computing.  Within this category, there are `rotated'~\cite{tomita2014low} and `unrotated'~\cite{fowler2012surface} variants. Rotated surface codes offer a higher resistance to errors and are somewhat less complex to implement than the unrotated versions thus, we focus exclusively on rotated surface codes in this work.

\subsection{Background and Motivation}

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{fig/basic.pdf}
    \caption{\textbf{Original and Modified Approaches in Rotated Surface Code}
     (a) A distance-3 and distance-5 rotated surface code layout, demonstrating the scalable structure of the code that enhances fault tolerance with increased distance. The layout shows how expanding the code distance, by adding additional qubits, increases robustness against errors.
     (b) Example of Z- and X-stabilizer circuits with ancilla measurements responsible for detecting bit-flip and phase-flip errors respectively.
     (c) Growth in qubit requirements with increasing code distance, illustrating the substantial overhead introduced by ancilla qubits. As the distance of the code increases to improve error tolerance, the number of qubits required for both data and ancilla qubits rises, with ancilla qubits contributing significantly to the total overhead.
     (d) Distance-3 rotated surface code shown over two rounds with decoding cycles.
     (e) Proposed approach of dividing each round into two sub-rounds, where ancilla qubits are repurposed. In this approach, the first sub-round measures only X-stabilizers, while the second sub-round measures only Z-stabilizers, using the same set of ancilla qubits. This strategy reduces the required number of ancilla qubits by half, effectively lowering the qubit overhead.
     (f) Modified surface code operation over two rounds, showing each round containing two sub-rounds and only one decoder after every complete round.
    }
    \label{fig:everything_basic}
    % \vspace{-20pt}
\end{figure*}

The structure of most quantum error-correcting codes (QECCs) is anchored in two main stabilizers: the X-stabilizer and the Z-stabilizer. X-stabilizers detect phase-flip (Z-flip) errors, while Z-stabilizers identify bit-flip (X-flip) errors. In Fig.~\ref{fig:everything_basic} \whitecircled{a}, a surface code with distance 3 is shown, illustrating how this layout works. Each ``distance" represents the code's error-tolerance level, with larger distances enhancing fault tolerance; this setup can scale to higher distances, such as distance 5, to increase robustness against errors.

The surface code is arranged on a d×d lattice, where each gray blob represents a data qubit. Every data qubit is monitored by both X and Z stabilizers, ensuring complete coverage for detecting both bit-flip and phase-flip errors. The green regions represent Z-stabilizers, while the blue regions indicate X-stabilizers. Ancilla qubits, used to capture error syndromes, are depicted as white blobs with borders: green-bordered white blobs for Z-stabilizers and blue-bordered white blobs for X-stabilizers.

In this arrangement, each stabilizer interacts with a set of four neighboring data qubits to generate a syndrome as shown in Fig.~\ref{fig:everything_basic} \whitecircled{b}. For example, a Z-stabilizer produces the syndrome $Z(q_0) \otimes Z(q_1) \otimes Z(q_2) \otimes Z(q_3)$, which is then projected onto an ancilla qubit. This projection yields a measurement $S_z$, indicating a $\pm 1$ outcome depending on the presence of a bit-flip error in the associated data qubits. Similarly, the X-stabilizer produces the syndrome $X(q_0) \otimes X(q_1) \otimes X(q_2) \otimes X(q_3)$ with the ancilla measurement $S_x$ indicating any phase-flip error. 

In this configuration, each stabilizer in the surface code has a corresponding ancilla qubit to capture its syndrome measurement—half of these stabilizers are designated as X-stabilizers, and the other half as Z-stabilizers. In a rotated surface code of distance \( d \), there are \( d^2 \) data qubits arranged in a \( d \times d \) grid. The stabilizers, which require ancilla qubits for syndrome measurement, are positioned both within the grid and along the boundaries. The number of squares (or cells) inside the grid that host stabilizers is \( (d - 1)^2 \), with each square containing either an X-stabilizer or a Z-stabilizer. Additionally, there are boundary stabilizers: \( d - 1 \) semi-circular X-stabilizers along the left and right edges and \( d - 1 \) semi-circular Z-stabilizers along the top and bottom edges. Summing these, the total number of stabilizers is \( (d - 1)^2 + 2(d - 1) = d^2 - 1 \). Therefore, \( d^2 - 1 \) ancilla qubits are needed to monitor these stabilizers. Combining the data and ancilla qubits, the total number of qubits in a rotated surface code of distance \( d \) is \( 2d^2 - 1 \). This result highlights the substantial resource demand from ancilla qubits in quantum error correction, as they are nearly equal in number to the data qubits, making efficient management of qubit overhead critical in scalable quantum computing. The total number of qubits required for a rotated surface code of distance \( d \) is given by: \( Q_{\text{total}} = 2d^2 - 1 \). Fig.~\ref{fig:everything_basic} \whitecircled{c} demonstrates the increase in data qubits as the distance of a rotated surface code is expanded. However, the overall rise in the total number of qubits is substantially greater, as this total includes both data and ancilla qubits. This difference underscores the significant resource demand imposed by the ancilla qubits, highlighting the importance of strategies to manage and reduce overall qubit overhead in scalable quantum error correction.

In a traditional implementation of the surface code, a single application of the code is insufficient for effective error correction. Instead, the surface code is applied repeatedly in sequential steps, known as rounds, on the same set of qubits. After each round, a decoding algorithm is executed to detect and correct errors based on the syndromes measured in that round. Once corrections are made, the process proceeds to the next round. This cycle can continue for as many rounds as needed to ensure stability and accuracy in the quantum computation. Fig.~\ref{fig:everything_basic} \whitecircled{d} shows a distance-3 rotated surface code running for two rounds, with decoding cycles at the end of each round.

\subsection{Contribution}

In this work, we introduce a modified approach to the surface code that significantly reduces the number of ancilla qubits without compromising the code's structural integrity or error-detection capabilities. Traditionally, a surface code round consists of a simultaneous measurement of both X-stabilizers and Z-stabilizers, each requiring a dedicated set of ancilla qubits. However, as depicted in Fig.~\ref{fig:everything_basic} \whitecircled{e}, we propose dividing each standard round into two sequential sub-rounds. In the first sub-round, only X-stabilizers are measured, utilizing a set of ancilla qubits. In the second sub-round, the same ancilla qubits are repurposed to measure Z-stabilizers. This reuse of ancilla qubits, marked by the purple circles in the figure, allows for a reduction in the number of ancilla qubits by half.

Fig.~\ref{fig:everything_basic} \whitecircled{f} illustrates the operation of our modified surface code over two full rounds. Each full round is divided into two sub-rounds: the first sub-round measures X-stabilizers, while the second sub-round measures Z-stabilizers, both utilizing the same set of ancilla qubits. The decoding algorithm is applied after each complete round to detect and correct any errors before moving on to subsequent rounds. This structure allows efficient reuse of ancilla qubits, reducing the total ancilla requirement while maintaining the integrity of error correction.

In this work, we modify the original approach to reduce the number of ancilla qubits while preserving the structure and integrity of the surface code. Specifically, we propose dividing a standard round of the surface code—typically comprising one set of X-stabilizer measurements and one set of Z-stabilizer measurements—into two half-rounds. In the first half, only X-stabilizers are measured, followed by a second half measuring only Z-stabilizers, reusing the same ancilla qubits employed for the X-stabilizers. This approach effectively reduces the number of required ancilla qubits by half.

In the original surface code configuration, each stabilizer (both X and Z) requires a separate ancilla qubit for syndrome measurement, resulting in a total of \( d^2 - 1 \) ancilla qubits for a code of distance \( d \). However, in our modified approach, we divide each round into two sub-rounds: one for X-stabilizer measurements and another for Z-stabilizer measurements. By reusing the same set of ancilla qubits across both types of stabilizers, we effectively reduce the number of required ancilla qubits by half. Thus, instead of needing \( d^2 - 1 \) ancilla qubits, our modified surface code requires only approximately \( \frac{d^2 - 1}{2} \) ancilla qubits. Thus, the reduction in the number of ancilla qubits \( R_{\text{ancilla}} \) is 50\%, which significantly lowers the overall resource demands of the code while preserving its error-correcting capabilities. In simple terms, the number of ancilla qubits is nearly equal to the number of data qubits in a traditional surface code. Thus, if we reduce the ancilla qubits by half, the total reduction in qubits should be close to 25\%. 

Fig.~\ref{fig:new_overhead_and_ratios} \whitecircled{a} compares four curves: ancilla qubits (original and the new approach) and total qubits (original and new). Both ancilla and total qubits increase with distance, but the new approach shows a marked reduction in ancilla qubits, leading to a corresponding decrease in the total qubit count. This indicates a significant reduction in qubit overhead when using recycled ancillas, especially as the distance increases. To prove this mathematically, we calculate the exact asymptotic reduction in the total number of qubits as \( d \) approaches a very large value. The reduction in the total number of qubits, \( R_{\text{total}} \), is calculated as:
\[
R_{\text{total}} = \frac{Q_{\text{original}} - Q_{\text{modified}}}{Q_{\text{original}}} \times 100\%.
\]

Substituting the values for \( Q_{\text{original}} = 2d^2 - 1 \) and \( Q_{\text{modified}} = \frac{3}{2}d^2 - \frac{1}{2} \):
\[
R_{\text{total}} = \frac{(2d^2 - 1) - \left(\frac{3}{2}d^2 - \frac{1}{2}\right)}{2d^2 - 1} \times 100\%.
\]

Now, simplify the numerator:
\[
R_{\text{total}} = \frac{2d^2 - 1 - \frac{3}{2}d^2 + \frac{1}{2}}{2d^2 - 1} \times 100\% = \frac{\frac{4d^2}{2} - \frac{3d^2}{2} - \frac{1}{2}}{2d^2 - 1} \times 100\%.
\]

Further simplifying, we get:
\[
R_{\text{total}} = \frac{\frac{d^2}{2} - \frac{1}{2}}{2d^2 - 1} \times 100\%.
\]

As \( d \) becomes large, To find the exact reduction in total qubits as, we take the limit of \( R_{\text{total}} \)

\[
\lim_{d \to \infty} R_{\text{total}} = \lim_{d \to \infty} \frac{\frac{d^2}{2} - \frac{1}{2}}{2d^2 - 1} \times 100\%.
\]

As \( d \to \infty \), the terms \(\frac{d^2}{2}\) in the numerator and \(2d^2\) in the denominator dominate, allowing us to approximate the reduction:

\[
\lim_{d \to \infty} R_{\text{total}} = \lim_{d \to \infty} \frac{\frac{d^2}{2}}{2d^2} \times 100\% = \frac{1}{4} \times 100\% = 25\%.
\]

This result shows that our modified surface code configuration not only reduces the number of required ancilla qubits by half but also achieves an approximate 25\% reduction in total qubits, making it a more resource-efficient approach to quantum error correction.

Fig.~\ref{fig:new_overhead_and_ratios} \whitecircled{b} plots the ratio of different types of qubits (ancilla to total and data to total) against the code distance, highlighting the proportion of each qubit type relative to the total count. In the new approach, the ``Ancilla to Total" ratio is noticeably lower. This reduction reflects the efficiency gained by reusing ancilla qubits, which lowers the overall qubit overhead. Conversely, the ``Data to Total" ratio increases in the new approach, indicating that data qubits now make up a larger proportion of the total qubits. This shift occurs not because of an increase in data qubits, but due to the reduced need for ancilla qubits. The increased proportion of data qubits suggests that the core structure of the code remains intact, preserving the code's error-correcting capability. By reducing ancilla overhead without impacting the number of data qubits, the new approach maintains 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{fig/new_overhead_and_ratios.pdf}
    \caption{\textbf{Comparison of Qubit Overhead and Ratios in Original and Modified Surface Code Approaches}
    (a) compares ancilla and total qubit requirements in the original and new approaches, showing that while both increase with code distance, the new approach achieves a marked reduction in ancilla qubits, leading to a lower total qubit count. This demonstrates the effectiveness of recycling ancillas to reduce overhead, particularly at higher distances.
    (b) shows the ratio of ancilla to total qubits and data to total qubits across different distances. The new approach has a noticeably lower ``Ancilla to Total" ratio, indicating increased efficiency through reduced ancilla usage. Meanwhile, the ``Data to Total" ratio increases in the new approach, confirming that the reduced need for ancilla qubits allows data qubits to make up a larger proportion of the total without compromising the integrity of the encoded data.
    }
    \label{fig:new_overhead_and_ratios}
    % \vspace{-20pt}
\end{figure}

\subsection{Parper Structure}

==> 3a_use_case_math.tex <==
\section{Illustrative Use Cases} \label{sec:use_case_math}

In practical applications of quantum error correction, users often face trade-offs between achieving a specific logical error rate and minimizing qubit overhead. The modified surface code offers a way to reduce the number of ancilla qubits required, making it a compelling choice in certain scenarios.

\subsection{Case 1: Relaxed Logical Error Rate Requirements}

Suppose a user needs to use a distance-3 surface code to achieve a target logical error rate. If the user can tolerate a slightly higher logical error rate than planned, they can switch to the modified method. This approach reduces the number of ancilla qubits by half, leading to approximately a 25\% reduction in total qubit overhead while still maintaining reasonable error-correcting capabilities.

To prove this mathematically, we calculate the exact asymptotic reduction in the total number of qubits as \( d \) approaches a very large value. The reduction in the total number of qubits, \( R_{\text{total}} \), is calculated as:
\[
R_{\text{total}} = \frac{Q_{\text{traditional}} - Q_{\text{modified}}}{Q_{\text{traditional}}} \times 100\%.
\]
Substituting the values for \( Q_{\text{traditional}} = 2d^2 - 1 \) and \( Q_{\text{modified}} = \frac{3}{2}d^2 - \frac{1}{2} \):
\[
R_{\text{total}} = \frac{(2d^2 - 1) - \left(\frac{3}{2}d^2 - \frac{1}{2}\right)}{2d^2 - 1} \times 100\%.
\]
% \[
% R_{\text{total}} = \frac{2d^2 - 1 - \frac{3}{2}d^2 + \frac{1}{2}}{2d^2 - 1} \times 100\% = \frac{\frac{4d^2}{2} - \frac{3d^2}{2} - \frac{1}{2}}{2d^2 - 1} \times 100\%.
% \]
% Further simplifying, we get:
\[
R_{\text{total}} = \frac{\frac{d^2}{2} - \frac{1}{2}}{2d^2 - 1} \times 100\%.
\]
As \( d \) becomes large, To find the exact reduction in total qubits as, we take the limit of \( R_{\text{total}} \)
\[
\lim_{d \to \infty} R_{\text{total}} = \lim_{d \to \infty} \frac{\frac{d^2}{2} - \frac{1}{2}}{2d^2 - 1} \times 100\% \sim 25\%
\]
% As \( d \to \infty \), the terms \(\frac{d^2}{2}\) in the numerator and \(2d^2\) in the denominator dominate, allowing us to approximate the reduction:
% \[
% \lim_{d \to \infty} R_{\text{total}} = \lim_{d \to \infty} \frac{\frac{d^2}{2}}{2d^2} \times 100\% = \frac{1}{4} \times 100\% = 25\%.
% \]
This result shows that our modified surface code configuration not only reduces the number of required ancilla qubits by half but also achieves an approximate 25\% reduction in total qubits, making it a more resource-efficient approach to quantum error correction. The modified approach offers an alternative to directly increasing the code distance, requiring fewer qubits than the traditional approach for achieving a similar or lower logical error rate. However, the user must have additional qubits in the system to implement the modified code.

\subsection{Case 2: Strict Logical Error Rate Requirements (\(d < 13\))}

In scenarios where the user aims to achieve the logical error rate associated with a surface code of distance \(d\) (original), using a modified surface code of the same distance will result in a slightly higher logical error rate. To meet the logical error rate requirement while reducing qubit overhead, the user can transition to a modified surface code of distance \(d + 2\).

The additional qubits required for this transition are calculated as:
\( \Delta Q = Q_{\text{modified}, d+2} - Q_{\text{traditional}, d}\).
Substituting the formulas for \(Q_{\text{modified}}\) and \(Q_{\text{traditional}}\), we obtain:
\[
\Delta Q = \left[ (d + 2)^2 + \frac{(d + 2)^2 - 1}{2} \right] - \left[ d^2 + (d^2 - 1) \right]
\]
\[
\Delta Q = \frac{1}{2}(d + 1)(13 - d)
\]

For distances \(d < 13\), this equation shows a \textbf{positive value of \(\Delta Q\)}, meaning the user will need \textbf{additional qubits} to transition from \(d\) (original) to \(d + 2\) (modified). However, this additional qubit requirement is less than what would have been needed to directly implement a surface code of distance \(d + 2\) (original). For instance, if \(d = 3\):
\[
Q_{\text{original}, d=3} = 3^2 + (3^2 - 1) = 17
\]
\[
Q_{\text{modified}, d+2=5} = 5^2 + \frac{(5^2 - 1)}{2} = 37
\]
\[
\Delta Q = 37 - 17 = 20
\]
In this example, the user needs 20 additional qubits to transition from \(d = 3\) (original) to \(d = 5\) (modified), achieving the logical error rate of a distance-5 code. This approach saves resources compared to directly implementing a distance-5 code (original), which would require 32 qubits instead of 37.

\subsection{Case 3: Resource-Efficient Transition (\(d \geq 13\))}

When the distance \(d\) (original) is large (\(d \geq 13\)), the situation changes significantly. From the formula:
\[
\Delta Q = \frac{1}{2}(d + 1)(13 - d)
\]
If \(d \geq 13\), the value of \(\Delta Q\) becomes \textbf{negative}, indicating that transitioning from \(d\) (original) to \(d + 2\) (modified) requires \textbf{fewer qubits}. This happens because the qubit-saving efficiency of the modified code at larger distances outweighs the additional resources needed for the increase in distance (as shown in Fig.~\ref{fig:new_overhead_and_ratios} \whitecircled{b}).
For example, if \(d = 13\):
\[
Q_{\text{original}, d=13} = 13^2 + (13^2 - 1) = 337
\]
\[
Q_{\text{modified}, d+2=15} = 15^2 + \frac{(15^2 - 1)}{2} = 337
\]
\[
\Delta Q = 337 - 337 = 0
\]
At \(d = 13\), the qubit requirements for \(d\) (original) and \(d + 2\) (modified) are identical.

For \(d > 13\), the modified code of \(d + 2\) requires \textbf{fewer qubits} than \(d\) (original). For instance, if \(d = 15\):
\[
Q_{\text{original}, d=15} = 15^2 + (15^2 - 1) = 449
\]
\[
Q_{\text{modified}, d+2=17} = 17^2 + \frac{(17^2 - 1)}{2} = 433
\]
\[
\Delta Q = 433 - 449 = -16
\]
In this case, transitioning from \(d = 15\) (original) to \(d = 17\) (modified) results in saving 16 qubits. The modified approach becomes even more efficient, enabling the user to achieve a similar or lower logical error rate of \(d + 2\) (modified) with \textbf{fewer qubits} than required for \(d\) (original). This makes the modified approach particularly advantageous for larger systems, where the savings in qubits can be significant.

\subsection{Case 4: Generalizing for What \(k\) Will \(d + k\) (Modified) Use Less Qubits Than \(d\) (Original)}

In this scenario, we determine how far a user can increase the distance \(k\) in a modified surface code (\(d + k\)) while using the same or fewer qubits than required for a distance \(d\) (original) surface code. This analysis highlights the flexibility of the modified surface code in leveraging additional error-correcting performance with fewer resources.

The total qubit count for a modified surface code of distance \(d + k\) is:
\(
Q_{\text{modified}, d+k} = (d + k)^2 + \frac{(d + k)^2 - 1}{2}
\); and the total qubit count for an original surface code of distance \(d\) is:
\(
Q_{\text{original}, d} = d^2 + (d^2 - 1)
\)
To find the maximum \(k\) for which the modified surface code uses the same or fewer qubits as the original, we solve the inequality:
\[
Q_{\text{modified}, d+k} \leq Q_{\text{original}, d}
\]
Substituting the formulas:
\[
(d + k)^2 + \frac{(d + k)^2 - 1}{2} \leq d^2 + (d^2 - 1)
\]
% \[
% \frac{3}{2}(d + k)^2 - \frac{1}{2} \leq 2d^2 - 1
% \]
% \[
% \frac{3}{2}(d + k)^2 \leq 2d^2 - \frac{1}{2}
% \]
% \[
% (d + k)^2 \leq \frac{4}{3}d^2 - \frac{1}{3}
% \]
\[
d + k \leq \sqrt{\frac{4}{3}d^2 - \frac{1}{3}}
\]
To approximate further, since \(\frac{4}{3}d^2 \gg \frac{1}{3}\), we can ignore \(\frac{1}{3}\) under the square root:
\[
d + k \leq \sqrt{\frac{4}{3}d^2} = \frac{2}{\sqrt{3}}d
\]
% Subtracting \(d\) from both sides:
% \[
% k \leq d \left(\frac{2}{\sqrt{3}} - 1\right)
% \]
Numerically, \(\frac{2}{\sqrt{3}} \approx 1.1547\), so:
\[
k \leq 0.1547d
\]

Let us calculate the maximum \(k\) for which a user can transition to \(d + k\) (modified) while using the same or fewer qubits as \(d = 27\) (original). Substituting \(d = 27\) into the formula:
\[
k \leq 0.1547 \cdot 27
\]
\[
k \leq 4.1769
\]
Since \(k\) must be an integer, \(k = 4\). This means a user currently using \(d = 27\) (original) can transition to \(d + 4 = 31\) (modified) while using the same or fewer qubits. We validate the above result by explicitly calculating the difference in total qubits (\(\Delta Q\)) for \(k = 4\) and \(k = 5\) to confirm the transition point.

For \(d = 27\) (original):
\[
Q_{\text{original}, d=27} = 27^2 + (27^2 - 1)= 1457
\]

For \(d + 4 = 31\) (modified):
\[
Q_{\text{modified}, d+4=31} = 31^2 + \frac{31^2 - 1}{2} = 1441
\]
\[
\Delta Q = Q_{\text{modified}, d+4=31} - Q_{\text{original}, d=27} = -16
\]
Since \(\Delta Q < 0\), \(d + 4 = 31\) (modified) uses fewer qubits than \(d = 27\) (original).


